Neural network scoring for efficient computing

Much work has been dedicated to estimating and optimizing workloads in high-performance computing (HPC) and deep learning. However, researchers have typically relied on few metrics to assess the efficiency of those techniques. Most notably, the accuracy, the loss of the prediction, and the computational time with regard to GPUs or/and CPUs characteristics. It is rare to see figures for power consumption, partly due to the difficulty of obtaining accurate power readings. In this paper, we introduce a composite score that aims to characterize the trade-off between accuracy and power consumption measured during the inference of neural networks. For this purpose, we present a new open-source tool allowing researchers to consider more metrics: granular power consumption, but also RAM/CPU/GPU utilization, as well as storage, and network input/output (I/O). To our best knowledge, it is the first fit test for neural architectures on hardware architectures. This is made possible thanks to reproducible power efficiency measurements. We applied this procedure to state-of-the-art neural network architectures on miscellaneous hardware. One of the main applications and novelties is the measurement of algorithmic power efficiency. The objective is to allow researchers to grasp their algorithms' efficiencies better. This methodology was developed to explore trade-offs between energy usage and accuracy in neural networks. It is also useful when fitting hardware for a specific task or to compare two architectures more accurately, with architecture exploration in mind.

==> preamble.tex <==
\IEEEoverridecommandlockouts
\RequirePackage[l2tabu,orthodox]{nag}     % Detect bad LaTeX
%\documentclass[a4paper,12pt]{article}
%\usepackage[a4paper,margin=2cm]{geometry}

\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}

\usepackage{mathtools,amsfonts}
\usepackage{url}
\usepackage[english]{babel}
\usepackage[final,activate=true,kerning=true,protrusion=true]{microtype}
\usepackage{enumerate}
\usepackage{tcolorbox}
\usepackage{graphicx}
\graphicspath{ {/} }
\usepackage{tabulary}
\usepackage{varioref}
\usepackage[pdfpagelabels=true]{hyperref}
\usepackage{cleveref}
\usepackage{xcolor}
\usepackage{booktabs}
\usepackage{csquotes}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\usepackage{stmaryrd} %For double brackets
\usepackage{eurosym}

\hypersetup{
	linktoc = page,
	pdfpagemode = UseNone,
	colorlinks,
	linkcolor={red!50!black},
	citecolor={blue!50!black},
	urlcolor={blue!80!black}
}

\pagestyle{plain}
\newcommand\tab[1][0.625cm]{\hspace*{#1}}
\usepackage{pgf,tikz}   %for Tikzfigures
\usepackage{pgfplots}
\usetikzlibrary{shapes,arrows,positioning}
\tikzstyle{decision} = [diamond, draw, text width=4.5em, text badly centered, node distance=5cm, inner sep=0pt]
\tikzstyle{block} = [rectangle, draw, text width=7.2em, text centered, rounded corners, minimum height=5em]
\tikzstyle{line} = [draw, -latex']
\tikzstyle{cloud} = [draw, ellipse, node distance=3cm, minimum height=2em]

%\usepackage[toc,page]{appendix}
\usepackage[style=ieee]{biblatex}
\bibliography{bibliography} 
\usepackage{amsmath}
\usepackage{caption}% <-- added
\captionsetup[table]{skip = 3pt}
\newcolumntype{L}{>{\raggedright\arraybackslash}X}% <-- added
\usepackage{ltablex}% <-- added
\usepackage{siunitx}% <-- added
\usepackage{stfloats}
\usepackage{comment}
%\usepackage{authblk}
\renewcommand{\ttdefault}{pcr} % selects Courier font

\usepackage{censor}
\usepackage{float} %<- Allows the use of [H] argument to prevent latex from repositionning figures
\usepackage{colortbl} %<- Allows cell coloring
\definecolor{lightblue}{rgb}{0.68, 0.85, 0.9} %<-Add lightblue coloring
\setlength{\textfloatsep}{0.1cm} %<- To ajust the space below tables
\setlength{\abovecaptionskip}{0.1cm} %<- To adjust the space over tables

